Visual onoma-to-wave: environmental sound synthesis from visual onomatopoeias and sound-source images

We propose a method for synthesizing environmental sounds from visually represented onomatopoeias and sound sources. An onomatopoeia is a word that imitates a sound structure, i.e., the text representation of sound. From this perspective, onoma-to-wave has been proposed to synthesize environmental sounds from the desired onomatopoeia texts. Onomatopoeias have another representation: visual-text representations of sounds in comics, advertisements, and virtual reality. A visual onomatopoeia (visual text of onomatopoeia) contains rich information that is not present in the text, such as a long-short duration of the image, so the use of this representation is expected to synthesize diverse sounds. Therefore, we propose visual onoma-to-wave for environmental sound synthesis from visual onomatopoeia. The method can transfer visual concepts of the visual text and sound-source image to the synthesized sound. We also propose a data augmentation method focusing on the repetition of onomatopoeias to enhance the performance of our method. An experimental evaluation shows that the methods can synthesize diverse environmental sounds from visual text and sound-source images.

==> fig/partitioning.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp3796101352946567] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (69.92,37.88) -- (329.92,37.88) -- (329.92,49.88) -- (69.92,49.88) -- cycle ;
%Shape: Rectangle [id:dp4918154254803251] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.54 ] (69.92,66.88) -- (170.92,66.88) -- (170.92,76.88) -- (69.92,76.88) -- cycle ;
%Shape: Rectangle [id:dp1263454580490353] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.56 ] (149.92,76.88) -- (260.92,76.88) -- (260.92,86.88) -- (149.92,86.88) -- cycle ;
%Shape: Rectangle [id:dp8775963547119923] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.55 ] (240.92,86.88) -- (329.92,86.88) -- (329.92,96.88) -- (240.92,96.88) -- cycle ;
%Straight Lines [id:da7856899965101948] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (69.92,27.88) -- (69.92,114.88) ;
%Straight Lines [id:da33561458894717244] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (160.92,44.88) -- (160.92,114.88) ;
%Straight Lines [id:da5346896577295797] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (250.92,43.88) -- (250.92,114.88) ;
%Straight Lines [id:da5540802931101504] 
\draw    (71.92,104.88) -- (158.92,104.88) ;
\draw [shift={(160.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(69.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da15822088877530105] 
\draw    (253.92,104.88) -- (328.92,104.88) ;
\draw [shift={(330.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(251.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da653467356994818] 
\draw    (162.92,104.88) -- (249.92,104.88) ;
\draw [shift={(251.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(160.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da21017878435256443] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (329.92,27.88) -- (329.92,114.88) ;
%Straight Lines [id:da640194301012043] 
\draw    (213.92,29.88) -- (327.92,29.88) ;
\draw [shift={(329.92,29.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da33763840313286453] 
\draw    (177.92,28.88) -- (71.92,28.88) ;
\draw [shift={(69.92,28.88)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da24706518655532705] 
\draw    (255.92,68.88) .. controls (256.88,49.58) and (266.23,56.36) .. (283.06,59.55) ;
\draw [shift={(284.92,59.88)}, rotate = 189.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10966678071540714] 
\draw    (250,69) -- (260.92,68.88) ;
\draw [shift={(260.92,68.88)}, rotate = 539.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;

% Text Node
\draw (104,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{cut}}$};
% Text Node
\draw (281,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{last}}$};
% Text Node
\draw (194,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{cut}}$};
% Text Node
\draw (187,20) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{full}}$};
% Text Node
\draw (286,53) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{overlap}}$};


\end{tikzpicture}


==> sec/conclusion_old.tex <==
\vspace{-2mm}
\section{Conclusion} \vspace{-2mm}\label{sec:conclusion}
    We proposed a method of constructing an audiobook speech corpus and constructed $31.5$ hours of data for Japanese audiobook speech synthesis. We evaluated the corpus in terms of audiobook speech synthesis and suggested factors for future direction of audiobook speech synthesis.
    
    J-MAC is open-sourced in our project page and is for research purpose only. The corpus does not include audio data, and users need to purchase the audiobook products from the websites listed in the corpus.

%%%% ASRU %%%%%
% In this paper, we propose a speech corpus construction strategy and build $1,300$ and $900$ hours data for Japanese ASR and ASV. First, we retrieved audio and subtitles from YouTube videos with manual subtitles. Then, we constructed corpora for ASR and ASV by CTC-based cleaning and speaker variation-based cleaning. One of our future directions is to extend the corpus to multiple languages. Our method (and open-sourced scripts) is almost language-independent, so it can be easily applied to languages other than Japanese. Another direction is the use of automatic subtitles, which are 45 times larger than manual subtitles.










==> sec/eval_old.tex <==
\vspace{-2mm}
\section{Proposed methods} \vspace{-2mm}\label{sec:experiment}
    \subsection{Evaluation in data collection} \vspace{-2mm}
        We crawled Audiobook.jp\footnote{\url{https://audiobook.jp}}, a largest audiobook provider in Japan, and prepared approximately 150 audiobooks. The reference text was crawled from Aozora Bunko\footnote{\url{https://www.aozora.gr.jp/}}, a Japanese digital library that stores out-of-copyright books. Texts of the books are provided in HTML format, and some characters (e.g., Chinese characters used in Japanese (kanji)) include reading aids. The structured text was automatically created from the HTML-format text. Chapter boundaries were signified with a chapter index or blank line. Boundaries of paragraphs, styles, and sentences were signified with indentations, quotation marks, and periods, respectively. The reading aids were also reflected in the structured text, e.g., kanji were accompanied with their readings. 

        \input{tab/method_expr_overall}

        \Table{corpus_spec} lists the specifications of our corpus. These values are not all the collected data described above but the actual corpus developed via the following experiments. From these values, we can describe 1) $1.9$ audiobooks were spoken per speaker, 2) $3.0$ audiobooks were collected per book, and $48.0$ minutes duration were collected per speaker. \Fig{fig/audiobook_statistics} shows histograms of audiobooks per book and speaker. We could collect audiobooks read by different speakers and those read by the same speaker. 

        \drawfig{t}{0.85\linewidth}{fig/audiobook_statistics}{Distribution of audiobooks per book (left) and speaker (right). Resulting corpus includes audiobooks read by different speakers and speaker who read multiple books.}

        \input{tab/corpus_comparison}

        \Table{corpus_comparison} compares J-MAC with the existing corpora. J-MAC is smaller than corpora of amateur speakers but has unique features: multiple professional speakers and parallel data (i.e., an audiobook spoken by different speakers). It is also the first open-source multi-speaker audiobook corpus in Japanese.
    
    \vspace{-2mm}    
    \subsection{Evaluation in background music estimation} \vspace{-2mm} % BGMを推定し，不要なものを削除
        We used a pre-trained model of Spleeter\footnote{\url{https://github.com/deezer/spleeter}} for deep learning-based vocal-instrumental separation. We used py-webrtcvad\footnote{\url{https://github.com/wiseman/py-webrtcvad}} for signal processing-based VAD.  

        \drawfig{t}{0.7\linewidth}{fig/snr}{SNR of each audiobook. Audiobooks are filtered on basis of manually determined threshold.}

        \Fig{fig/snr} shows the results of SNR calculation. The SNR ranged from $0$~dB (i.e., voices and instrumentals are similar in volume.) to $100$~dB (very clean). The threshold was determined manually because it was difficult to determine it automatically due to its gentle variation. The ``Clean'' audiobooks proceeded to segmentation, as described in the next subsection.
    
    \vspace{-2mm}
    \subsection{Evaluation in segmentation} \vspace{-2mm}% ASR と VAD の話．
        We used an recurrent neural network (RNN)-based CTC alignment model provided by ESPnet~\cite{watanabe18espnet}. The model was trained using the CSJ corpus~\cite{maekawa00csj}. The CTC score improvement by re-alignment converged until three iterations. The $5$-best sentences on the CTC scores were used to split audio in re-alignment. 
    
        \drawfig{t}{0.7\linewidth}{fig/ctc}{CTC scores of each audiobook. Re-alignment improves CTC score. Audiobooks with lower CTC scores are eliminated.}
        \drawfig{t}{0.7\linewidth}{fig/vad_shift}{Distribution of VAD-based timing refinement. Both start and end timings given by CTC-based alignment have offsets and are refined by VAD.}
        
        \Fig{fig/ctc} shows the CTC scores. The re-alignment significantly improved the CTC scores around $-4.0$--$-2.0$ and contributed to selecting more well-aligned audiobooks. Even after realignment, the CTC scores of certain audiobooks were significantly lower ($< -4.0$). We examined these audiobooks and found that they were translations of Japanese books into English. Although the text and audio do not basically correspond, some named entities do (e.g., readings of the main character's name in Japanese text is represented in English speech). The interesting finding is that these alignments did not fail, and CTC scores are obtained.     
        
        \Fig{fig/vad_shift} shows histograms of timing shift by VAD. Most of the aligned timings were shifted, suggesting that CTC alignment alone can result in overlapping in the speech segment; our correction using VAD avoids this problem.
        
    \vspace{-2mm}
    \subsection{Evaluation in speech synthesis} \vspace{-2mm}
        Finally, we evaluated our corpus on an audiobook speech synthesis task using multiple synthesis methods, audiobooks, and speakers. We trained a multi-speaker speech synthesis model and evaluated the synthetic speech of different books and speakers.
    
        \subsubsection{Model setup}
            % nakata-kun
            % speech synthesis setup
            
            \drawfig{t}{0.98\linewidth}{fig/architecture}{Architectures of audiobook speech synthesis. Left considers only current sentence as well as basic text-to-speech, and right considers neighboring sentences. In practice, subsequent sentences are also taken into account, but for simplicity, only preceding sentences are input into BERT in right figure.}
            
            % \begin{figure*}[t]
            %     \centering
            %     \subfigure[Model architecture of SingleSentence]{
            %         \includegraphics[clip,height=0.242\linewidth]{fig/model/SingleSentence}}
            %     \subfigure[Model architecture of MultiSentences]{
            %         \includegraphics[clip,height=0.242\linewidth]{fig/model/MultiSentences}}
            %     % \subfigure[Architecture of variance adaptor]{
            %     %     \includegraphics[clip,height=0.198\linewidth]{fig/model/VarianceAdaptor}}
            %     \caption{Model architecture of SingleSentence and MultiSentences. The gray box indicates model input and output. When concatenating feature from BERT output, the embedding is duplicated by the phoneme count to match the length.}
            %     \label{fig:speech_synthesis_model}
            % \end{figure*}
            % \begin{figure}
            %     \centering
            %     \includegraphics[clip,height=0.484\linewidth]{fig/model/VarianceAdaptor}
            %     \caption{Architecture of variance adaptor}
            %     \label{fig:variance Adaptor}
            % \end{figure}
            
            %To evaluate the corpus on the speech synthesis task, we used a modified version of SingleSentence and MultiSentences\cite{nakata21_ssw}.
            %The modified version of the model is based on FastSpeech2~\cite{ren2021fastspeech} instead of Tacotron2\cite{shen18tacotron2} and the sentence-level embedding was used instead of word-level embedding. 
            %\Fig{fig/architecture} shows the model architecture of the modified version of SingleSentence and MultiSentences.
            %SingleSentence takes the current sentence to be synthesized into account while MultiSentences takes the current sentence and its neighboring sentences into account. In this work, a total of 500 tokens (previous sentences + current sentence + following sentences) were extracted from the corpus for each sample. 
            %This enables the MultiSentences to capture cross-sentence context while SingleSentence cannot.
            We used a modified version of Nakata's method~\cite{nakata21_ssw}, which retrieves contexts of input text using bidirectional encoder representations from Transformers (BERT)~\cite{vaswani17allYouNeed}. \Fig{fig/architecture} shows the model architecture. The ``SingleSentence'' method synthesizes speech sentence by sentence in isolation, as with the basic reading-style speech synthesis. The ``MultiSentences'' method synthesizes speech of the current sentence, using neighboring sentences (previous, current, and following sentences). The modified version of the model was based on FastSpeech2~\cite{ren2021fastspeech} instead of Tacotron2~\cite{shen18tacotron2}, and sentence-level embedding was used instead of word-level embedding. This enables MultiSentences to capture cross-sentence context while SingleSentence cannot. To train on a multi-speaker corpus, speaker lookup embedding was used. 
            
            %In our implementation, the variance adaptor is composed of pitch predictor, energy predictor and duration predictor. The pitch and energy predictor predicts by phoneme-level instead of frame-level. The pitch and energy were extracted by frames and averaged over each phoneme duration. To train on multi-speaker corpus, speaker lookup embedding was used. The output of speaker embedding was added to encoder output along with the sentence-level feature from BERT.
            % Moreover, Postnet composed of 1-D convolution layers are applied to decoder output to boost the synthesized speech quality.
            
            % For dataset, We used J-MAC. All samples were downsampled to 22.05~kHz, segmented into a sentence level and split into train/validation set in advance. The size of train/validation set is 14043/100 samples respectively. Julius \cite{lee09julius} was used to get alignments between utterances and phoneme sequences. The generated melspectrogram configurations were 80 dimensions, with the frame length of 1024 samples and frame shift of 256 samples.  
            We downsampled audio data to $22.05$~kHz, segmented them into a sentence level, and split them into training and validation sets in advance. The sizes of the training and validation sets were $14,043$ and $100$ samples, respectively. Julius~\cite{lee09julius} was used to obtain alignments between utterances and phoneme sequences. The generated melspectrogram configurations were 80 dimensions, with frame length of $1,024$ samples and frame shift of $256$ samples.
            
            % As for the BERT model, we used small BERT configuration to save computational resources.
            %Our BERT model was pretrained on Japanese Wikipedia with model configuration of 2 Transformer layers, 2 attention heads, 512 intermediate state size and 128  hidden state size. This model configuration is equivalent to BERT-tiny which is proposed on \cite{turc2019wellread}. However, we did not perform pretrained distillation. 
            We used the pre-trained BERT model trained using Japanese Wikipedia data. The model configuration is equivalent to BERT-tiny~\cite{turc2019wellread}. However, we did not perform pre-trained distillation. The BERT weights are unfreezed upon training except for the embedding layer as not all vocabulary appear on the training set. 
            
            For optimization, we used the Adam optimizer with $\beta_1 = 0.9$, $\beta_2 = 0.99$. Learning rate scheduling was applied in the same manner as in a previous study~\cite{vaswani17allYouNeed} with $4,000$ warmup steps, and the batch size was 64. For the loss function, we used the mean square error of each output from a variance adapter and the melspectrogram of the model output and decoder output (i.e. output before going through Postnet). The BERT weights are unfreezed upon training except for the embedding layer as not all vocabulary appear on the training set. We used HiFiGAN~\cite{kong20hifigan} with the weights distributed on official code implementation\footnote{\url{https://github.com/jik876/hifi-gan}}. Specifically, we used the UNIVERSAL\_V1 model. We did not perform finetuning of the HiFiGAN parameters.
            
        \subsubsection{Results and analysis of subjective evaluation}
            We conducted a mean opinion score (MOS) evaluation on the naturalness of audiobook speech. We explored the effect of speaker, book, and synthesis method on naturalness. Under these conditions, we synthesized audiobook speech in paragraph level containing 2--5 sentences. Six speakers (3 males and 3 females labeled ``m1''--``f3'') were randomly selected from the corpus. The test set was four audiobooks ("akai", "akazukin", "donguri", and "tsuchigami," which are labeled ``book1''--``book4,'' respectively) selected from the J-KAC corpus~\cite{nakata21_ssw}. The test set had no overlap from the training and validation sets, but all the sets belonged to the same domain of books (all were developed from the same source (Aozora Bunko)). 260 listeners participated to the MOS test and each listener evaluated randomly selected 10 samples.   
            
            \Table{mos} lists the MOS score under each condition. From these results, we can provide the following insights.
            \begin{itemize} \itemsep 0mm \leftskip -5mm 
                \item \textbf{Synthesis method}: Considering multiple sentences slightly improves naturalness ($3.24$ vs. $3.30$) in audiobook speech synthesis.
                \item \textbf{Books}: The naturalness significantly changes by book ($3.01$--$3.45$). As mentioned above, the domains of these books and the training data are the same, so factors other than the domain affect the scores. 
                \item \textbf{Speakers}: The naturalness also changes by speaker ($2.97$--$3.43$). The amount of training data for the low-scoring speakers ``m2'' and ``m3'' (2 and 4 audiobooks, respectively) is more than those for ``m1'' and ``m3'' (1 audiobook, respectively), so we cannot say that the reason for this result is the amount of training data alone.
            \end{itemize}

            % MOS result
            \input{tab/mos}
      
            \Table{statistics} shows the results of the analysis of variance (ANOVA). Statistical significance was observed in each of synthesis method, book, and speaker. These results also indicate that there is an interaction among each factor, except for between method and speaker. This suggests that a synthesis method using multiple sentences improves naturalness to the same extent regardless of speaker, and that there is an entanglement between synthesis methods, speakers, and books, and that this disentanglement is necessary to improve the quality of audiobook speech synthesis. These will be good directions for audiobook speech synthesis research using this corpus.

            % ANOVA result
            \input{tab/statistics}
            
        
        




%%%% ASRU %%%%
%     \subsection{Evaluation in data collection}
%         The video data was collected between February and April of 2021. Also, the Wikipedia timestamp used to create search terms was February 2021. \Table{corpus_spec} lists the number of search terms and videos we collected. From these numbers, we can describe that
%             \begin{itemize} \leftskip -5mm
%                 \item $5.09$ videos are found for each search term.
%                 \item $0.92$~\% of videos have manual subtitles, and $41.7$~\% have automatic subtitles.
%             \end{itemize}
            
%         In the end, we obtained approximately 10,000 hours of speech data from 110,000 YouTube videos. \Fig{fig/duration} shows duration of videos and utterances. Most of the videos are less than 5 minutes long, and the average duration is 3.8 minutes. Also, a few videos are several hours long but these are very rare. On the other hand, almost all utterances are shorter than 25 seconds because the subtitles are synchronized with the video, but a few utterances are several hours long. 
        
%         \input{tab/corpus_spec}
%         \input{tab/corpus_comparison}

%         \drawfig{t}{0.9\linewidth}{fig/duration}
%         {Duration of found videos and its statistics.}

%         \Table{corpus_comparison} shows a comparison with the existing corpus. The duration of our corpus is not all of the collected data described above but subsets used in the ASR and ASV experiments described below. Among ASR corpora, our corpus is similar in size to LaboroTVspeech (Japanese)~\cite{ando21laborotvspeech} and Common Voice (English)~\cite{ardila20commonvoice}. Also, among ASV corpora, it is the first open-source Japanese corpus and is similar in size to CN-Celeb (Chinese)~\cite{fan19cnceleb}. We are planning to further analyze the collected data and expand the corpus size.

%     \subsection{Evaluation in speech recognition}
%         \subsubsection{Data cleaning}
%         \label{sec:data_cleaning}
%         The most important data pre-processing is to prune utterances that have the wrong transcriptions and fix the incorrect timing.
%         We consistently employed CTC segmentation and CTC scoring, as described in Section \ref{sec:ctc_score_seg}.
%         We used a pre-trained CTC model based on the ESPnet LaboroTVspeech~\cite{ando21laborotvspeech} recipe\footnote{\url{https://github.com/espnet/espnet/tree/master/egs2/laborotv/asr1}}. 
%         Table \ref{tab:asr_data_stats} summarizes the statistic of the various training and test sets.
        
%         As a pilot study, we used two subsets of our corpus:
%         \begin{itemize}
%             \item "single\_speaker" (or "ss" in short): based on the single speaker subset, as described in Section \ref{sec:asv}
%             \item "top\_15k" (or "15k" in short): extracted based on top 15,000 videos in terms of the average score for each video.
%         \end{itemize}
%         The total file size of the single\_speaker and top\_15k subsets including the silence region amounts to 100GB and 300GB, respectively.
%         Note that top\_15k is cleaned only based on utterance confidence scores and it may contain multi speaker videos, unlike single\_speaker.
%         Also these subsets are overlapped.
        
%         \drawfig{t}{0.85\linewidth}{fig/hist_score_L20}
%         {Histograms of the score for different ASR models over all utterances of top\_15k, with a scoring length that corresponds to $0.96$s of audio.}

%         These subsets are further decomposed into the training and test sets, which will be explained in the next section.
%         We also prepare the various training sets by changing the threshold value $\theta$ of the confidence score obtained by CTC segmentation for the single\_speaker and top\_15k subsets.
%         To determine the threshold value, we investigate the distribution of the confidence score over all utterances in the top\_15k subset, as shown in \Fig{fig/hist_score_L20}.
%         This distribution clearly shows that the peak of the distribution starts around -3.0 in both RNN and transformer based CTC models.
%         Based on the observation, we regard the utterances located in the wide-based region as outlier data points, and use -3.0 as the lowest threshold for pruning in Table~\ref{tab:asr_data_stats}.
        
%         The largest training set is obtained by combining the single\_speaker and top\_15k subsets (train\_ss\_15k).
%         It contains more than 17 thousand videos, 1.2 million utterances, and 1.3 thousand hours\footnote{We can further scale up our training data up to approximately five times more if we use the entire corpus.}.
        
%         \subsubsection{Test set design}
%         \label{sec:test_set_design}
%         We carefully designed a test set for ASR evaluation from our corpus.
%         First, we only focused on the "single\_speaker" videos to reduce the cost of manual process of verifying the audio and corresponding correct transcriptions.
%         The rest of the procedure is as follows:
%         \begin{enumerate}
%             \item Select 1,621 videos from the "single\_speaker" videos that include "easy" utterances scored more than -0.3 threshold value based on CTC.
%             \item Randomly pick up 324 videos (around 20\%) and use them as a test video set, which has 3,396 easy utterances in total.
%             \item Manually listen utterances and identify 1,614 utterances having correct transcriptions.
%             \item Split them into the development (\textbf{dev\_easy\_jun21}) and evaluation (\textbf{eval\_easy\_jun21}) sets, which have 785 and 829 utterances, respectively.
%         \end{enumerate}
%         We also made an additional test set with "normal" utterances\footnote{
%         The definition of "easy" and "normal" test sets are determined based on the CTC score objectively. Our listening process and later ASR experiments confirmed that this categorization is reasonable.
%         } scored more than $-1.0$ threshold value.
%         We fixed to use the same test video set as we defined before, and performed steps 3 and 4.
%         We made \textbf{dev\_normal\_jun21} and \textbf{eval\_normal\_jun21} sets, which have 1,036 and 834 utterances, respectively.
%         We will perform the above procedure for the different threshold value or non single\_speaker subsets to create more difficult (e.g., hard) test sets in the future.

% \begin{table}[t]
%     \centering
%     \caption{Training and test data statistics for the ASR task. $\theta$ is a threshold value used to prune bad utterances based on the CTC score.}
%     \label{tab:asr_data_stats}
%     \begin{tabular}{c|rrrr}
%     & $\theta$ & \# videos & \# utts & hours \\
%     \hline
%     dev\_easy\_jun21       & -0.3 & 110   & 785     & 0.7 \\
%     eval\_easy\_jun21      & -0.3 & 106   & 829     & 0.7 \\
%     dev\_normal\_jun21     & -1.0 & 128   & 1,036   & 1.1 \\
%     eval\_normal\_jun21    & -1.0 & 129   & 834     & 0.8 \\
%     \hline
%     train\_single\_speaker & -0.3 & 1,297 & 14,797  & 12.7 \\
%     train\_single\_speaker & -0.5 & 1,792 & 26,209  & 24.2 \\
%     train\_single\_speaker & -1.0 & 2,906 & 66,563  & 71.9 \\
%     train\_single\_speaker & -2.0 & 4,068 & 186,733 & 227.4 \\
%     train\_single\_speaker & -3.0 & 4,342 & 285,846 & 362.0 \\
%     \hline
%     train\_top\_15k & -3.0 & 14,418 & 1,048,699 & 1087.1 \\
%     \hline
%     train\_ss\_15k & -3.0 & 17,761 & 1,270,124 & 1376.9 \\
%     \end{tabular}
% \end{table}

%         \subsubsection{ASR models}
%         We used an ESPnet state-of-the-art conformer model \cite{gulati20conformer,guo2021recent} based on hybrid CTC/attention architectures \cite{watanabe20202020}.
%         The conformer encoder has 12 conformer blocks with 31 kernel size, 512 attention dimensions, 8 attention heads, and 2,048 feed forward dimensions.
%         The transformer encoder has 8 self attention blocks with 512 attention dimensions, 8 attention heads, and 2,048 feed forward dimensions.
%         We used SpecAugment during training \cite{park2019specaugment}.
%         We did not use LM shallow fusion during inference.
%         The detailed configuration can be found in the ESPnet JTubeSpeech recipe\footnote{\url{https://github.com/espnet/espnet/pull/3311}}.

%         \subsubsection{Experimental results}
%         \Fig{fig/cer_hour} shows the ASR performance for various amounts of the single\_speaker training data by changing the score threshold $\theta$.
%         We used the easy and normal test sets, as described in Section \ref{sec:test_set_design}, and the figure shows that the normal test set was more difficult than the easy test set (the error rate was increased by 1.6 to 2.1 times more).
%         This increase of the error rates validates our design of the test set by controlling the difficulties based on the score.
%         As regards the various amounts of the single\_speaker training data, if we increase the amount of training data by reducing the CTC score threshold, the training data may contain more noisy transcriptions or distorted audio segments.
%         Nevertheless, the ASR performance was improved as we increased the amount of training data.
%         The final CERs were $5.2\%$ in eval\_easy\_jun21 and $10.7\%$ in eval\_normal\_jun21.
%         These CER ranges are similar to the other Japanese ASR benchmarks, e.g., $4-6\%$ in CSJ \cite{maekawa00csj} and $13\%$ in LaboroTVspeech \cite{ando21laborotvspeech}.
%         Thus, we can conclude that our ASR benchmark is reasonable as our initial step of the corpus design.
        
%         We also list the largest training data case (ss\_15k\_1376h) in \Fig{fig/cer_hour}.
%         This data was obtained by combining the single\_speaker subset and the top\_15k subset, which contains multi-speaker recordings, as described in Section \ref{sec:data_cleaning}. 
%         Although the performance of the dev\_easy\_jun21 was degraded possibly due to the mismatch between single speaker and multi-speaker recordings, the performance of the normal test set was improved.
%         The eval\_normal\_jun21 CER was improved from $10.7\%$ to $10.0\%$.
%         This result shows that while we need more careful cleaning if we want to maintain the clean speech recognition task performance, more training data would be generally helpful to improve the performance of more challenging data.
        
%     \drawfig{t}{1.05\linewidth}{fig/cer_hour}
%     {ASR performance for various amounts of training data (12, 24, 71, 227, 362, and 1376 hours) by changing the score threshold and combining multi-speaker recordings. See Table \ref{tab:asr_data_stats} for the detailed training data information.} 
    
%         Finally, we evaluate the effectiveness of CTC segmentation, as discussed in Section \ref{sec:ctc_score_seg}.
%         We used train\_single\_speaker with $-1.0$ score threshold (71.9 hours) and prepared the corresponding training data based on the original YouTube timings only with CTC scoring.
%         Table \ref{tab:ctc_seg} shows that the CTC segmentation significantly improved the performance and shows the effectiveness of the re-aligning for the YouTube audio data, as suggested by \cite{chen2021gigaspeech}.
    
% \begin{table}[t]
%     \centering
%     \caption{The effectiveness of CTC segmentation.}
%     \label{tab:ctc_seg}
% \begin{tabular}{l|cr|cr}
%                                  & \multicolumn{2}{c|}{dev}                               & \multicolumn{2}{c }{eval}                            \\
%                                  & easy                     & \multicolumn{1}{c|}{normal} & easy                    & \multicolumn{1}{c}{normal} \\ \hline
% \multicolumn{1}{r|}{original timing} & \multicolumn{1}{r}{11.5} & 16.5                        & \multicolumn{1}{r}{9.2} & 15.7                       \\
% \multicolumn{1}{r|}{CTC segmentation}  & \multicolumn{1}{r}{\textbf{9,2}}  & \textbf{14.3}                       & \multicolumn{1}{r}{\textbf{6.9}} & \textbf{13.6}                      
% \end{tabular}
% \end{table}    
    
 


%     \subsection{Evaluation in speaker verification}
%         \subsubsection{Data cleansing}
%         We used py-webrtcvad\footnote{\url{https://github.com/wiseman/py-webrtcvad}} for VAD and an open-sourced pre-trained model\footnote{\url{https://github.com/yistLin/dvector}} for extracting $d$-vectors. The intra-video variation in speaker space was computed from more than 10 utterances for each video. As a pilot study, we used randomly selected 35,000 videos (approx. 30\% of total).
        
%         \Fig{fig/tsne_score_rev} shows the log determinant of a covariance matrix of $d$-vectors in each video (i.e., intra-video variation). In this figure, we can see two levels of rapid increase. The first level is near 0 on the x-axis, which means that videos with extremely low variance are included in the collected data. The second level is near 8 to 9 on the x-axis. Following the concept in \Fig{fig/single-speaker-collection}, we set a threshold around these levels and assign ``TTS,'' ``single speaker,'' or ``multi speakers,'' class to the videos, starting from the lowest value.
    
%         \drawfig{t}{0.85\linewidth}{fig/tsne_score_rev}
%         {Log determinant of covariance matrix of $d$-vectors in each video}    

%         We quantitatively evaluate the authenticity of this classification. We randomly extracted 100 videos from each class and annotated a true class label. In the annotation, multi-TTS videos (i.e., multiple TTS systems are used in the video) and overdubbed-voice videos (e.g., overdubbed singing voices) were annotated as ``multi speakers.'' To accurately find TTS videos, a speech synthesis specialist participated in this annotation.

%         \Table{video_type} lists the result. It is observed that each class has their suitable videos. Especially, the ``single speaker'' class does not have multi-speaker videos. Therefore, we can demonstrate that our method works for eliminating the multi-speaker videos and choosing the single-speaker videos. Some single-speaker videos leak to the ``TTS'' class, but this impact is limited because the ``TTS'' class has only a few videos.

%         \input{tab/video_type}

%         \subsubsection{ASV dataset design}
%         For considering the usage of the same evaluation sets as ASR, we designed the evaluation trials from the ASR evaluation set (\textbf{eval\_easy\_jun21)}.  From the single-speaker evaluation set, 92 unique speakers were selected as the enrollment and testing speakers. Then, we selected 1,795 unique speakers for a training dataset and development one from the single-speaker videos except for the videos of the 92 speakers. Consequently, 3498 videos were used for training and development datasets. For the training, we cut each video by simple VAD, then, 127,997 and 25,392 utterances were used for training and development datasets, respectively. 
%         In the testing, we designed an enrollment utterance and a testing one were picked up from the same video but different time. For picking up the test utterances accurately, the manual subtitle information was used. In the testing, we performed 25,392 trial pairs, included 276 correct pairs and 25,116 incorrect pairs.

%         \subsubsection{ASV models}      
%         We used a speaker embedding network, which was built with four convolutional neural networks, pooling layers and two full connected layers. The output of the final layer was regarded as a speaker embedding vector. As the input feature, 40-order Mel-Frequency Cepstrum Coefficients with 25-ms frame length and half overlapped shift were used. The speaker-embedding vector was 512 dimensions. The speaker embedded vectors extracted from the enrollment utterances and the testing utterance were compared by the cosine distance similarity. Equal error rate (EER) was used for our evaluation.

%         \subsubsection{ASV performance}
%         We performed ASV evaluations, and the EER of our ASV system with JTubeSpeech was \textbf{10.9\%}.  Our system was regarded as the speaker embedding system based on the CNN-based model and evaluated with the cosine distance similarity. Even though such a simple system, this result had the similar performance to the CNN-based model (VGG-M) trained with Voxceleb1~\cite{nagrani19voxceleb}.
%         As a pilot study, we designed a simple benchmark. For example, the result was obtained with the small model and probabilistic linear discriminant analysis (PLDA) scoring and data augmentation techniques were not performed. And, since the trial pairs of the correct cases were picked up from the same video in the correct pair cases, some trial part seemed to be easy. However, from this simple benchmark, we could show the techniques of data cleaning for selecting a unique speakers and 
%         constructing ASV systems performed well. Consequently, we established the Japanese ASV systems with large-scale open source media in the first time.
% %        because of the dataset came from Youtube videos, there were hevy BGM and sound effects. The 
        

% %        Table \ref{tab:asv_results} shows the EER of our ASV system with JTubeSpeech. As a pilot study, we designed a simple benchmark. For example, the result was obtained with a small model and probabilistic linear discriminant analysis (PLDA) scoring and data augmentation techniques were not performed. Since the trial pairs were picked up from the same video in the correct pair cases, some part seemed to be easy.         
%         To fully utilize YouTube videos for estimating reliable ASV systems, data augmentation and speech enhancement techniques and other data cleaning schemes will be required. In addition, as shown in Table \ref{tab:video_type}, some TTS speakers remained in the single speakers dataset. We will discuss the influences of including TTS speakers and how to eliminate such speakers. To keep the reproducibility of our ASV system, we will add the ASV recipe based on the ESPnet style in the future.

% \begin{comment}
%     \begin{table}[t]
%         \centering
%         \caption{EER (\%) of ASV evaluation.}
%         \label{tab:asv_results}
%         \begin{tabular}{c|r}
%         & eval\_easy\_jun21  \\
%         \hline
%         Spk embeddings / cosine dist. & 10.9\% 
%         \end{tabular}
%     \end{table}  
% \end{comment}
        
    

==> tab/method_expr_overall.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\vspace{-1mm}
\centering
\caption{Corresponding table of experiments and methods in each subsection. Two types of models trained with sound event images were prepared: one using photographs and the other using line drawings.}
\footnotesize
\begin{tabular}{cccc||cccc}
\multicolumn{4}{c||}{Method}                                                                                                                                                                                                                                                        & \multicolumn{4}{c}{Experiment}                                                            \\ \hline
\multicolumn{1}{c|}{}                                                                                      & \begin{tabular}[c]{@{}c@{}}Sound\\ event\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Data\\ aug.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Img\\ str.\end{tabular} & 4.2.1                & 4.2.2                & 4.2.3                & 4.2.4                \\ \hline
\multicolumn{1}{c|}{Reconstraction}                                                                        & \multicolumn{1}{l}{}                                       & \multicolumn{1}{l}{}                                & \multicolumn{1}{l||}{}                              & \CheckmarkBold       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \CheckmarkBold \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Onoma-to-wave}}                                                        & label                                                      &                                                     &                                                   & \CheckmarkBold       & \CheckmarkBold       &                      &                      \\
\multicolumn{1}{c|}{}                                                                                      & label                                                      & \CheckmarkBold                                      &                                                    &                      & \CheckmarkBold       &                      &                      \\ \hline
\multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Image-aware \\ Onoma-to-wave \\ (proposed)\end{tabular}}} & label                                                      &                                                     &                                                    & \CheckmarkBold       & \CheckmarkBold       &                      & \CheckmarkBold       \\
\multicolumn{1}{c|}{}                                                                                      & label                                                      & \CheckmarkBold                                      &                                                    &                      & \CheckmarkBold       & \CheckmarkBold       &                      \\
\multicolumn{1}{c|}{}                                                                                      & label                                                      & \CheckmarkBold                                      & \CheckmarkBold                                     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \CheckmarkBold       & \multicolumn{1}{l}{} \\
\multicolumn{1}{c|}{}                                                                                      & \begin{tabular}[c]{@{}c@{}}Photo\end{tabular}   &                                                     &                                                    &                      &                      &                      & \CheckmarkBold       \\
\multicolumn{1}{c|}{}                                                                                      & \begin{tabular}[c]{@{}c@{}}Line drawing\end{tabular} &                                                     &                                                    &                      &                      &                      & \CheckmarkBold       \\ 
\end{tabular}
\vspace{-3mm}
\label{tab:methods}
\end{table}
